ZeroLeak: Using LLMs for Scalable and Cost Effective Side-Channel Patching

Security critical software, e.g., OpenSSL, comes with numerous side-channel leakages left unpatched due to a lack of resources or experts. The situation will only worsen as the pace of code development accelerates, with developers relying on Large Language Models (LLMs) to automatically generate code. In this work, we explore the use of LLMs in generating patches for vulnerable code with microarchitectural side-channel leakages. For this, we investigate the generative abilities of powerful LLMs by carefully crafting prompts following a zero-shot learning approach. All generated code is dynamically analyzed by leakage detection tools, which are capable of pinpointing information leakage at the instruction level leaked either from secret dependent accesses or branches or vulnerable Spectre gadgets, respectively. Carefully crafted prompts are used to generate candidate replacements for vulnerable code, which are then analyzed for correctness and for leakage resilience. From a cost/performance perspective, the GPT4-based configuration costs in API calls a mere few cents per vulnerability fixed. Our results show that LLM-based patching is far more cost-effective and thus provides a scalable solution. Finally, the framework we propose will improve in time, especially as vulnerability detection tools and LLMs mature.

==> TODO.tex <==
Experiments:

1- Scan all libraries in the Javascript table.

2- Use Spectector or something else to try fixing Spectre gadgets.

3- Use LLaMa-2 Huggingface models to compare the performance with GPT-4.

4- Make a table for C functions. We can still use Microwalk for that.

5- Can we find another tool instead of Microwalk for comparison?




==> misc/result.tex <==
{
    "CallStack": [
        {
            "CallStackId": "B72012A755DB1563",
            "SourceInstructionImageName": "target-microbenchmark",
            "SourceInstructionOffset": "0x166c",
            "SourceInstructionFormatted": "target-microbenchmark:TraceFunc+1f9",
            "TargetInstructionImageName": "target-microbenchmark",
            "TargetInstructionOffset": "0x16ca",
            "TargetInstructionFormatted": "target-microbenchmark:RunTarget+0",
            "LeakageEntries": [],
            "Children": [
                {
                    "CallStackId": "D89FCBBF161F2432",
                    "SourceInstructionImageName": "target-microbenchmark",
                    "SourceInstructionOffset": "0x1a19",
                    "SourceInstructionFormatted": "target-microbenchmark:RunTarget+34f",
                    "TargetInstructionImageName": "target-microbenchmark",
                    "TargetInstructionOffset": "0x1200",
                    "TargetInstructionFormatted": "target-microbenchmark:_init+200",
                    "LeakageEntries": [
                        {
                            "ImageName": "libleaky_functions.so",
                            "Offset": "0x1ad5",
                            "Type": "jump",
                            "NumberOfCalls": 1,
                            "TreeDepth": {
                                "Mean": 5.0,
                                "StandardDeviation": 0.0,
                                "Minimum": 5,
                                "Maximum": 5
                            },
                            "MutualInformation": {
                                "Mean": 1.88,
                                "StandardDeviation": 0.0,
                                "Minimum": 1.88,
                                "Maximum": 1.88
                            },
                            "ConditionalGuessingEntropy": {
                                "Mean": 0.75,
                                "StandardDeviation": 0.0,
                                "Minimum": 0.75,
                                "Maximum": 0.75,
                                "Score": 103.33,
                                "ScoreStandardDeviation": 0.0
                            },
                            "MinimumConditionalGuessingEntropy": {
                                "Mean": 1.0,
                                "StandardDeviation": 0.0,
                                "Minimum": 1.0,
                                "Maximum": 1.0,
                                "Score": 100.0,
                                "ScoreStandardDeviation": 0.0
                            }
                        },
                        {
                            "ImageName": "libleaky_functions.so",
                            "Offset": "0x1aef",
                            "Type": "jump",
                            "NumberOfCalls": 2,
                            "TreeDepth": {
                                "Mean": 4.5,
                                "StandardDeviation": 0.5,
                                "Minimum": 4,
                                "Maximum": 5
                            },
                            "MutualInformation": {
                                "Mean": 1.29,
                                "StandardDeviation": 0.16,
                                "Minimum": 1.12,
                                "Maximum": 1.45
                            },
                            "ConditionalGuessingEntropy": {
                                "Mean": 0.75,
                                "StandardDeviation": 0.12,
                                "Minimum": 0.62,
                                "Maximum": 0.88,
                                "Score": 103.33,
                                "ScoreStandardDeviation": 1.67
                            },
                            "MinimumConditionalGuessingEntropy": {
                                "Mean": 1.0,
                                "StandardDeviation": 0.0,
                                "Minimum": 1.0,
                                "Maximum": 1.0,
                                "Score": 100.0,
                                "ScoreStandardDeviation": 0.0
                            }
                        },
                        {
                            "ImageName": "libleaky_functions.so",
                            "Offset": "0x1b09",
                            "Type": "jump",
                            "NumberOfCalls": 4,
                            "TreeDepth": {
                                "Mean": 3.0,
                                "StandardDeviation": 1.0,
                                "Minimum": 2,
                                "Maximum": 4
                            },
                            "MutualInformation": {
                                "Mean": 0.72,
                                "StandardDeviation": 0.05,
                                "Minimum": 0.62,
                                "Maximum": 0.75
                            },
                            "ConditionalGuessingEntropy": {
                                "Mean": 0.33,
                                "StandardDeviation": 0.21,
                                "Minimum": 0.19,
                                "Maximum": 0.69,
                                "Score": 108.96,
                                "ScoreStandardDeviation": 2.79
                            },
                            "MinimumConditionalGuessingEntropy": {
                                "Mean": 1.0,
                                "StandardDeviation": 0.0,
                                "Minimum": 1.0,
                                "Maximum": 1.0,
                                "Score": 100.0,
                                "ScoreStandardDeviation": 0.0
                            }
                        }
                    ],
                    "Children": []
                }
            ]
        }
    ]
}

==> misc/test.tex <==
#include <stdint.h>
#include <string.h>
#include <stdlib.h>
#include <stdio.h>
#include <stdbool.h>
#include <assert.h>
#include "../src/leaky_functions.c"
//***************************************************************************
void test_memory_leakage_case_1() {
  assert(memory_leakage_case_1(1, 2, 1) == 2);
}

void test_memory_leakage_case_2() {
  assert(memory_leakage_case_2(2) == 144);
}

void test_memory_leakage_case_3() {
  assert(memory_leakage_case_3(7) == 41);
}

void test_memory_leakage_case_4() {
  uint8_t msg[16] = {0};
  uint8_t msg2[16] = {49, 56, 48, 57, 54, 55, 53, 50, 51, 52, 49, 56, 48, 57, 54, 55};
  for (int i = 0; i < 16; i++) {
    msg[i] = 48 + (i*7+17)%10;
  }
  memory_leakage_case_4(msg, 16);
  assert(memcmp(msg, msg2, 16) == 0);
  
}

void test_memory_leakage_case_5() {
  assert(memory_leakage_case_5(13) == 13);
}

//***************************************************************************

void test_branch_leakage_case_1() {
  char pw[16] = "abcdabcdabcdabcd";
  char in[16] = "abcdabcdabcdabcd";
  char in2[16] = "abdabdasdasdasdg";
  assert(branch_leakage_case_1(pw, in) == 1);
  assert(branch_leakage_case_1(pw, in2) == 0);

}

void test_branch_leakage_case_2() {
  uint8_t a[16] = {15, 14, 13, 12, 11, 10, 9, 8, 7, 6,
       5, 4, 3, 2, 1, 0};
  uint8_t a2[16] = {0, 1, 2, 3, 4, 5, 6, 7, 8, 9,
       10, 11, 12, 13, 14, 15};
  branch_leakage_case_2(a, 16);
  for (int i = 0; i < 16; i++) {
    assert(a[i] == a2[i]);
  }
}

void test_branch_leakage_case_3() {
  char p[3] = "abc";
  char q[3] = "abc";
  char p2[3] = "bbd";
  assert(branch_leakage_case_3(p, q) == 1);
  assert(branch_leakage_case_3(p, p2) == 0);

}

void test_branch_leakage_case_4() {
  assert(branch_leakage_case_4(0, 20) == 20);
  assert(branch_leakage_case_4(1, 20) == 0);
}

void test_branch_leakage_case_5() {
  assert(branch_leakage_case_5(5, 2) == 0);
  assert(branch_leakage_case_5(0, -2) == 5);
  assert(branch_leakage_case_5(-5, 0) == 1);

}

void test_branch_leakage_case_6() {
  assert(branch_leakage_case_6(1) == 11);
}

void test_branch_leakage_case_7() {
  assert(branch_leakage_case_7(1, 2, 1) == 2);
}
//***************************************************************************

int main() {
  test_memory_leakage_case_1();
  test_memory_leakage_case_2();
  test_memory_leakage_case_3();
  test_memory_leakage_case_4();
  test_memory_leakage_case_5();

  test_branch_leakage_case_1();
  test_branch_leakage_case_2();
  test_branch_leakage_case_3();
  test_branch_leakage_case_4();
  test_branch_leakage_case_5();
  test_branch_leakage_case_6();
  test_branch_leakage_case_7();

  printf("All tests passed successfully!\n");
  return 0;
}


==> misc/ubench.tex <==
#include <stdint.h>
#include <string.h>
#include <stdlib.h>
#include <stdio.h>
#include <stdbool.h>

//////////////////////////////////////////////////////////////////////////////////////
//////////////////////////////////////////////////////////////////////////////////////
// taken from https://github.com/PLSysSec/haybale-pitchfork
int memory_leakage_case_1(int x, int y, int option) {
    volatile int z[3] = { 0, 2, 300 };
    z[2] = y;
    if (option > 3) {
        return z[1];
    } else {
        return z[x % 3];
    }
}
// table lookup - taken from DATA - https://www.usenix.org/system/files/conference/usenixsecurity18/sec18-weiser.pdf
unsigned char LUT[16]={0x52, 0x19, 0x3E, 0x7F,
                    0x0C, 0x5A, 0x6D, 0x2B,
                    0x3F, 0x1A, 0x7E, 0x53, 
                    0x6C, 0x5B, 0x0D, 0x37};
int memory_leakage_case_2_transform(int kval) { return LUT[kval % 16]; }
int memory_leakage_case_2(int key){
    int val = memory_leakage_case_2_transform(0);
    val+=memory_leakage_case_2_transform(key);
    return val;
}

// from cached paper  - https://www.usenix.org/system/files/conference/usenixsecurity17/sec17-wang-shuai.pdf
int memory_leakage_case_3(int secret){
    int table[128] = {0};
    for (int i=0; i<128; i++){
        table[i] = i;
    }
    int i, t;
    int index = 0;
    for (i=0; i<200; i++){
        index = (index+secret) % 128;
        t = table[index];
        t = table[(index) % 79];
    }
    return t;
}

const uint8_t book[10] __attribute__((aligned(64))) = { 52, 48, 55, 51, 56, 54, 50, 49, 57, 53 };
uint8_t* memory_leakage_case_4(uint8_t* msg, unsigned len) {
for (unsigned i = 0; i < len; ++i)
    msg[i] = book[msg[i]-48];

return msg;
}

// getelement - taken from CacheAudit https://www.usenix.org/system/files/conference/usenixsecurity13/sec13-paper_doychev.pdf
unsigned int A[16] = {0, 1, 2, 3, 4, 5, 6, 7,
                      8, 9, 10, 11, 12, 13, 14, 15};
int memory_leakage_case_5(int secret) {
    if (secret < 16)
        return A[secret];
}
//////////////////////////////////////////////////////////////////////////////////////
//////////////////////////////////////////////////////////////////////////////////////

// isDiffVul1 - taken from FlowTracker https://dl.acm.org/doi/pdf/10.1145/2892208.2892230
int branch_leakage_case_1(char *pw, char *in) {
 int i;
 for (i=0; i<16; i++) {
    if (pw[i]!=in[i]) {
        return 0;
    }
 }
 return 1;
}

// InsertionSort - taken from CacheAudit https://www.usenix.org/system/files/conference/usenixsecurity13/sec13-paper_doychev.pdf
uint8_t * branch_leakage_case_2(uint8_t *a, int array_size){
    int i, j, index;
    for (i = 1; i < array_size; ++i){
        index = a[i];
        for (j = i; j > 0 && a[j-1] > index; j--)
            a[j] = a[j-1];
        a[j] = index;
    }

return a;

}


// eq - Time variant - taken from FlowTracker https://dl.acm.org/doi/pdf/10.1145/2892208.2892230
int branch_leakage_case_3(char *p, char *q) {
 if (p[0] != q[0])
    return false;
 else if (p[1] != q[1])
    return false;
 else
    return p[2] == q[2];
} 

// example 1 - taken from Blazer https://dl.acm.org/doi/pdf/10.1145/3062341.3062378
// This program takes a secret input high, and an attackercontrolled (tainted) input, low. A program is said to have a
// timing channel if the attacker, assumed to know the program
// code, can infer information about the high by observing
// the program’s running time (perhaps iteratively varying the
// input low). 
int branch_leakage_case_4(int high, uint low) {
    int i;
    if (high == 0) {
        i = 0;
        while(i < low) i++;
    }
    else {
        i = low;
        while(i > 0) i--;
    }
    return i;
}

// example 2 - taken from Blazer https://dl.acm.org/doi/pdf/10.1145/3062341.3062378
int branch_leakage_case_5(int high, int low) {
    int i;
    if (low > 0) { // O(2*low)
        i = 0;
        while(i<low) i++;
        while(i>0) i--;
    } else { // O(1)
        if (high == 0) { i = 5; } 
        else { i = 0; i++; }
    }
    return i;
}

// taken from https://github.com/PLSysSec/haybale-pitchfork
int branch_leakage_case_6(int x) {
    if (x > 10) {
        return x % 200 * 3;
    } else {
        return x + 10;
    }
}

// taken from https://github.com/PLSysSec/haybale-pitchfork
int branch_leakage_case_7(int x, int y, int option) {
    volatile int z[3] = { 0, 2, 300 };
    z[2] = y;
    if (option > 3) {
        return z[1];
    } else {
        return z[2];
    }
}

// from ctgrind tool  github repo
char branch_leakage_case_8(unsigned char *a, unsigned char *b) {
  unsigned i;
  for (i = 0; i < 16; i++) {
    if (a[i] != b[i])
      return 0;
  }

  return 1;
}

// mu - taken from SC-Eliminator https://dl.acm.org/doi/pdf/10.1145/3213846.3213851
// "the C code of a textbook implementation of a 3-way cipher,
// where the variable a is marked as secret and it affects the execution
// time of the if-statements. By observing the timing variation, an
// adversary may be able to gain information about the bits of a.""
int32_t * branch_leakage_case_9(int32_t *a) {
    int i;
    int32_t b[3];
    b[0] = b[1] = b[2] = 0;
    for (i=0; i<32; i++) {
        b[0] <<= 1; 
        b[1] <<= 1; 
        b[2] <<= 1;
        if(a[0]&1) 
            b[2] |= 1;
        if(a[1]&1) 
            b[1] |= 1;
        if(a[2]&1) 
            b[0] |= 1;
        a[0] >>= 1; 
        a[1] >>= 1; 
        a[2] >>= 1;
    }
    a[0] = b[0]; 
    a[1] = b[1]; 
    a[2] = b[2];

return a;
}

// taken from https://github.com/PLSysSec/haybale-pitchfork
uint8_t branch_leakage_case_10(uint8_t* public_arr, uint8_t public_arr_len, uint8_t* secret_arr, uint8_t i) {
    uint8_t x = public_arr[i];
    for (int j = 0; j < public_arr_len; j++) {
        secret_arr[j] += x;
    }
    if (x > 10) {
        return public_arr[0] + secret_arr[0];
    } else {
        return public_arr[1] + secret_arr[1];
    }
}

// bubblesort- taken from CacheAudit https://www.usenix.org/system/files/conference/usenixsecurity13/sec13-paper_doychev.pdf
uint8_t * branch_leakage_case_11(uint8_t *a, int n){
    int i, j, temp;
    for (i = 0; i < n - 1; ++i)
        for (j = 0; j < n - 1 - i; ++j)
            if (a[j] > a[j+1]){
                temp = a[j+1];
                a[j+1] = a[j];
                a[j] = temp;
            }
    return a;
 }


// SelectionSort - taken from CacheAudit https://www.usenix.org/system/files/conference/usenixsecurity13/sec13-paper_doychev.pdf
uint8_t * branch_leakage_case_12(uint8_t *a, int array_size){
    int i;
    for (i = 0; i < array_size - 1; ++i){
        int j, min, temp;
        min = i;
        for (j = i+1; j < array_size; ++j){
            if (a[j] < a[min])
                min = j;
        }
        temp = a[i];
        a[i] = a[min];
        a[min] = temp;
    }
    return a;
}


//////////////////////////////////////////////////////////////////////////////////////
//////////////////////////////////////////////////////////////////////////////////////
